Logarithmic Regret and Polynomial Scaling in Online Multi-step-ahead Prediction

This letter studies the problem of online multi-step-ahead prediction for unknown linear stochastic systems. Using conditional distribution theory, we derive an optimal parameterization of the prediction policy as a linear function of future inputs, past inputs, and past outputs. Based on this characterization, we propose an online least-squares algorithm to learn the policy and analyze its regret relative to the optimal model-based predictor. We show that the online algorithm achieves logarithmic regret with respect to the optimal Kalman filter in the multi-step setting. Furthermore, with new proof techniques, we establish an almost-sure regret bound that does not rely on fixed failure probabilities for sufficiently large horizons $N$. Finally, our analysis also reveals that, while the regret remains logarithmic in $N$, its constant factor grows polynomially with the prediction horizon $H$, with the polynomial order set by the largest Jordan block of eigenvalue 1 in the system matrix.

==> Preamb.tex <==
\usepackage[font=small]{caption}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage[normalem]{ulem}   
\usepackage{bm}
\usepackage{algorithm} 
\usepackage{algorithmic}
\usepackage{comment}
\usepackage[hidelinks]{hyperref}
\usepackage{xcolor}
\definecolor{subsectioncolor}{RGB}{0,0,128}   

\usepackage{balance} 
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{bbold}
\usepackage{mathtools}
\usepackage{tcolorbox}
\usepackage{bbm}
\usepackage{todonotes}
\usepackage{tensor}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}

\let\labelindent\relax
\usepackage{enumitem} 
\setlist{nolistsep,leftmargin=*,labelindent=0pt}
\usepackage{threeparttable}


\newcommand{\poly}{\operatorname{poly}}
\newcommand{\trace}{\operatorname{tr}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\tr}{\mathsf{ T}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\Sym}{\mathbb{S}}


\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}%[section]
\newtheorem{invariant}[theorem]{Invariant}
\newtheorem{remark}{Remark}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}{Proposition}%[section]
\newtheorem{corollary}{Corollary}%[section]
\newtheorem{example}{Example}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}{Assumption}%[section]
\newtheorem{fact}{Fact}


\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}


\newcommand{\innerproduct}[2]{\left \langle #1, #2 \right\rangle }
\newcommand{\Fnorm}[1]{\|#1\|_{\mathrm{F}}}

\definecolor{moccasin}{rgb}{0.98, 0.92, 0.84}
\newtcolorbox{mybox}{colback=moccasin,
colframe=moccasin}

\usepackage[nameinlink]{cleveref}

\crefname{theorem}{Theorem}{Theorems}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{example}{Example}{Examples}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{proposition}{Proposition}{Propositions}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{section}{Section}{Sections}
\crefname{appendix}{Appendix}{Appendices}
\Crefname{theorem}{Theorem}{Theorems}
\Crefname{corollary}{Corollary}{Corollaries}
\Crefname{example}{Example}{Examples}
\Crefname{lemma}{Lemma}{Lemma}
\Crefname{proposition}{Proposition}{Propositions}
\Crefname{figure}{Figure}{Figures}
\Crefname{table}{Table}{Tables}
\Crefname{section}{Section}{Sections}
\Crefname{appendix}{Appendix}{Appendices}


\newcommand{\sn}{\mathbb{S}^n}
\newcommand{\snp}{\mathbb{S}^n_+}
\newcommand{\snn}{\mathbb{S}^n_-}
\newcommand{\psolution}{\Omega_{\mathrm{P}}}
\newcommand{\dsolution}{\Omega_{\mathrm{D}}}






